Exploring physics beyond the Standard Electroweak Model in the light of supersymmetry

In this thesis we try to discuss certain phenomenological aspects of an R-parity violating non-minimal supersymmetric model, called $\mu\nu$SSM. We show that $\mu\nu$SSM can provide a solution to the $\mu$-problem of supersymmetry and can simultaneously accommodate the existing three flavour global data from neutrino experiments even at the tree level with the simple choice of flavour diagonal neutrino Yukawa couplings. We show that it is also possible to achieve different mass hierarchies for light neutrinos at the tree level itself. In $\mu\nu$SSM, the effect of R-parity violation together with a seesaw mechanism with TeV scale right-handed neutrinos are instrumental for light neutrino mass generation. We also analyze the stability of tree level neutrino masses and mixing with the inclusion of one-loop radiative corrections. In addition, we investigate the sensitivity of the one-loop corrections to different light neutrino mass orderings. Decays of the lightest supersymmetric particle were also computed and ratio of certain decay branching ratios was observed to correlate with certain neutrino mixing angle. We extend our analysis for different natures of the lightest supersymmetric particle as well as with various light neutrino mass hierarchies. We present estimation for the length of associated displaced vertices for various natures of the lightest supersymmetric particle which can act as a discriminating feature at a collider experiment. We also present an unconventional signal of Higgs boson in supersymmetry which can lead to a discovery, even at the initial stage of the large hadron collider running. Besides, we show that a signal of this kind can also act as a probe to the seesaw scale. Certain other phenomenological issues have also been addressed.

==> TexFilesW/style2N.tex <==
% Last modified by PRADIPTA on 17 JUNE, 2011
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% USEAPCKAGE {OPTIONS} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{phdthesis}
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{cite}
\usepackage{xcolor}
\usepackage{hyperref}
\hypersetup{colorlinks, linkcolor={blue}}
%\usepackage{hyperref}
%\usepackage{psboxit}
%\PScommands
\usepackage{fancyhdr}
\usepackage{amsmath}
%\usepackage{draftwatermark}
\usepackage{geometry}
\geometry{%
  textwidth  = 156mm ,
  textheight = 234mm ,
  a4paper            ,
  includehead        ,
  hcentering         ,
  vcentering
}
\usepackage{textcomp}
\usepackage[printwatermark]{xwatermark}
%\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{lipsum}

\newwatermark[allpages,color=gray!25,angle=45,scale=2.5,xpos=0,ypos=0]{ \textcopyright \sf PRADIPTA GHOSH}
%\usepackage{fancybox}
%\usepackage[options]{titlepage_melbourne_uni}
%\usepackage[options]{titlepage_melbourne_uni2}
%\usepackage{notes2bib}
%\usepackage{mciteplus}
%\usepackage{hyperref}
%%%%%%%%%%%%%%  LAYOUT  %%%%%%%%%%%%%%%%%%%%%%%%%%
%\oddsidemargin = 0.42in
%\evensidemargin = 0.1in
%\textwidth = 6.1in
%\headheight = 0in
%\headsep = 0in
%\topmargin = -0.2in
%\textheight = 9.0in
%\textwidth=17cm 
%\textheight=22.5cm 
%\oddsidemargin -0.65cm 
%\topmargin -1.5cm 
\renewcommand{\baselinestretch}{1.2}
%\renewcommand{\baselinestretch}{1.29}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% now change the section heading to have a line beneath it
%% load up the fancy title-style package
\RequirePackage[calcwidth]{titlesec}
\titleformat{\section}[hang]{\sffamily\bfseries}
{\Large\thesection}{12pt}{\Large}[{\titlerule[0.5pt]}]
%% now redefine the plain style pages (chapter pages, contents pages)
%% to have the same page number stuff on the bottom
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%  DEFINATIONS  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\rpv{\not\!\!{R_p}}
\def\L{\not\!\!{L}}
\def\D{\not\!\!{D}}
\def\k{\not\!\!{k}}
\def\a{\not\!\!{a}}
\def\b{\not\!\!{b}}
\def\ptmiss{\not\!\!{p_T}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
%\def\href{\hyperref}
\def\lam{\lambda}
\def\kp{\kappa}
\def\ovl{\overline}
\def\wt{\widetilde}
\def\al{\alpha}
\def\del{\delta}
\def\ep{\epsilon}
\def\pl{\partial}
\def\rt2{\sqrt{2}}
\def\nn{\nonumber}
\def\vp{\varepsilon}
\def\bN{\mathbf N}
\def\bU{\mathbf U}
\def\bV{\mathbf V}
\def\bRs{\mathbf R^{S^0}}
\def\bRp{\mathbf R^{P^0}}
\def\bRc{\mathbf R^{S^{\pm}}}
\def\Rs{R^{S^0}}
\def\Rp{R^{P^0}}
\def\Rc{R^{S^{\pm}}}
\def\Rsq{\mathbf R^{\widetilde q}}
\def\Rsu{\mathbf R^{\widetilde u}}
\def\Rsd{\mathbf R^{\widetilde d}}
\def\Ru{\mathbf R^{u}}
\def\Rd{\mathbf R^{d}}
\def\B{\mathbf B}
\def\q{\widetilde q}
\def\u{\widetilde u}
\def\d{\widetilde d}
\def\ntrli{\widetilde{\chi}^0_i}
\def\ntrlj{\widetilde{\chi}^0_j}
\def\n{{\widetilde \chi}^0}
\def\ps{\displaystyle{\not} p}
\def\qs{\displaystyle{\not} q}
\def\as{\displaystyle{\not} a}
\def\ntrli{\widetilde{\chi}^0_i}
\def\ntrlj{\widetilde{\chi}^0_j}
\def\tg{\widetilde g}
\newcommand{\usq}[1]{\widetilde{u}_#1}
\newcommand{\dsq}[1]{\widetilde{d}_#1}
\newcommand{\csq}[1]{\widetilde{c}_#1}
\newcommand{\ssq}[1]{\widetilde{s}_#1}
\newcommand{\bsq}[1]{\widetilde{b}_#1}
\newcommand{\tsq}[1]{\widetilde{t}_#1}
\newcommand{\ns}[1]{S^0_#1}
\newcommand{\nps}[1]{P^0_#1}
\newcommand{\cs}[1]{S^\pm_#1}
\newcommand{\ntrl}[1]{\widetilde{\chi}^0_#1}
\newcommand{\chpm}[1]{\widetilde{\chi}^{\pm}_#1}
\def\gsim{\lower0.5ex\hbox{$\:\buildrel >\over\sim\:$}}
\def\lsim{\lower0.5ex\hbox{$\:\buildrel <\over\sim\:$}}
\def\A{\.{A}}
%\def\lsim{\mathrel{\mathpalette\@versim<}}
%\def\gsim{\mathrel{\mathpalette\@versim>}}
%\def\gsim{\lower0.5ex\hbox{$\:\buildrel >\over\sim\:$}}
%\usepackage[calcwidth]{titlesec}
%\titleformat{\section}[hang]{\sffamily\bfseries}
% {\Large\thesection}{12pt}{\Large}[{\titlerule[0.5pt]}]

